Outer Billiards and the Pinwheel Map

In this paper we establish a kind of bijection between the orbits of a polygonal outer billiards system and the orbits of a related (and simpler to analyze) system called the pinwheel map. One consequence of the result is that the outer billiards system has unbounded orbits if and only if the pinwheel map has unbounded orbits. As the pinwheel map is much easier to analyze directly, we think that this bijection will be helpful in attacking some of the main questions about polyonal outer billiards.

==> 4broad.tex <==

\section{The Proof in Broad Strokes}

\subsection{The Exit Map}
\label{swap}

We fix a nice polygon $P$ for the entire chapter.
We define
$\widehat \psi(p)=\psi^k(p)$, where $k$ is the smallest
positive integer such that $p$ and $\psi^k(p)$ lie in
different tiles in the forward partition.
We call $\widehat \psi$ the {\it exit map\/}.
It is an immediate consequence of
Lemma \ref{exit} that $\widehat \psi=\psi$ on
the union of the bounded tiles in the forward
partition.  We introduce $\widehat \psi$ so
as to deal with all the tiles in the forward
partition in a uniform way.

\begin{lemma}
\label{replace}
Let $\Sigma$ be a pinwheel strip.  There exists a
compact subset $K \subset \Sigma$ with the following
property.  If $p \in \Sigma-K$ and
$\psi^k(p) \in \Sigma-K$, then we have
$\psi^k(p) = (\widehat \psi)^h(p)$ for some positive $h$.
\end{lemma}

\startproof
Without loss of generality we assume that $\Sigma=\Sigma_1$.
Let $p_j=\psi^j(p)$.  If we choose the compact set $K$
large enough, we can guarantee that
$p_{k-1}$ lies in the unbounded tile corresponding
to the strip $\Sigma_0$ and $p_k$ lies in the
unbounded tile corresponding to $\Sigma_1$.
We just choose $K$ as in the previous section.

We call $p_j$ {\it distinguished\/}
if $p_{j-1}$ and $p_j$ belong to different tiles in
the forward partition.   We also call $p_0=p$ distinguished.
Let $\widehat p_j$ denote the $j$th distintuished point.
By definition of $\widehat \psi$, we have
$$\widehat \psi(\widehat p_j)=\widehat p_{j+1}.$$
If we choose $K$ large enough, then
$p_{k-1}$ lies in the
unbounded tile $T(1 \to 1)$ whereas $p_k \in T(2 \to 2)$.
Hence $p_k$ is distinguished.   That is,
$p_k=\widehat p_h$ for some positive $h$. But then
$$p_k=\widehat \psi^h(\widehat p_0)=\widehat \psi^h(p),$$
as desired.
\endproof

In light of Lemma \ref{replace}, it suffices to prove
the Pinwheel Theorem for $\widehat \psi$ in place of
$\psi$.  



\subsection{Two Structural Results}

In this section we collect the $2$ main ingredients
we use in the proof of the Pinwheel Theorem.
As in Figure 2.6, we label the admissible
paths by their starting
and ending spokes.  

For any indices $a,b \in \{1,...,n\}$ we
define $b'$ to be the smallest integer
such that $b' \equiv b$ mod $n$ and
$a \leq b'$.  Then we define
\begin{equation}
M(a \to b) = \mu_{b'} \circ  \ldots  \circ \mu_a.
\end{equation}
Every strip map $\mu_i$ occurs in this composition,
for $i=a,...,b'$, and $\mu_{k+n}=\mu_k$. 
We also define  
\begin{equation}
\Sigma(a \to b) = \bigcap_{k=a}^{b'-1} \Sigma_i; \hskip 40 pt
\Sigma(a \to a) = \R^2.
\end{equation}
In case $a=b$ the second definition is meant to override
the first one.

We have already seen that the tiles in the forward partition
are labelled by the admissible paths.  We let
$T(a \to b)$ denote the tile labelled by the path
$a \to b$.  In case $a=b$, the set $T(a \to a)$ will
denote the union of the two unbounded tiles corresponding
to the spoke $a$.


We prove the following structure result
in \S \ref{proof3}.  This result
is meant to hold for all pairs 
tiles in the forward partition.

\begin{theorem}
\label{structure3}
$\widehat \psi(T(a \to b)) \cap T(c \to d) \subset \Sigma(b \to c).$
\end{theorem}

We prove the following structure result
in \S \ref{proof2}.  This result
is meant to hold for any tile
in the forward partition.

\begin{theorem}
\label{structure2}
$\psi=M(1 \to b)$ on the interior of 
any bounded tile $T(1 \to b)$.
\end{theorem}

The next result works for arbitrary tiles
in the forward partition.

\begin{corollary}
\label{structure22}
$\widehat \psi=M(a \to b)$ on the interior of 
$T(a \to b)$.
\end{corollary}

\startproof
For unbounded tiles in the forward partition,
Corollary \ref{structure22} follows immediately
from our analysis in \S \ref{easy}.
On bounded tiles, we have
$\widehat \psi = \psi$, so Corollary \ref{structure22}
follows from Theorem \ref{structure2}.
\endproof


\subsection{A Correspondence of Orbits}
\label{ocl}

We will work with the strip $\Sigma_1$.
We start with a point $p_1$ having the following properties.
\begin{itemize}
\item $p_1$ has a well-defined $\widehat \psi$-orbit.
\item $p_1 \in \Sigma_1$.
\item $p_1$ lies in the unbounded tile $T(2 \to 2)$.
\end{itemize}
We let $q_0=p_0$ and recursively define
\begin{equation}
p_{j+1}=\widehat \psi(p_j).
\hskip 30 pt
q_{j+1} = \mu_j(q_j).
\end{equation}

All numbers in the next lemma
are positive integers, and $n$ denotes
the number of sides of our nice polygon $P$.

\begin{lemma}
\label{orbit}
The following two statements are true.
\begin{itemize}
\item For any $k_1$ there is a 
$k_2$ such that $q_{k_2}=p_{k_1}$.
\item For any $k_2'$ there are
$k_1$ and $k_2$ such that
$q_{k_2}=p_{k_1}$ and $k_2 \leq k_2'<k_2+2n$.
\end{itemize}
\end{lemma}

\startproof
Let
\begin{equation}
T_j=T(a_j \to b_j)
\end{equation}
be the tile in the forward partition
such that $p_j \in T_j$.
Let 
\begin{equation}
M_j=M(a_j \to b_j).
\end{equation}
To make our argument go more smoothly, we take
indices mod $n$ and arrange
that 
$$2=a_1 = b_1 \leq a_2 \leq b_2 \leq a_3 \leq b_3 \ldots$$
We choose our indices to be as small as possible, so that
the difference between successive indices is at most $n-1$.
We define the map
\begin{equation}
M^*_{j+1}=\mu_{a_{j+1}-1} \circ  \cdots \circ \mu_{b_j+1} \circ \mu_{b_j}.
\end{equation}

\noindent
{\bf Remark:\/}
In terms of the notation above, we night say that
$M^*_{j+1} = M(a_{j+1}-1 \to b_j)$, but
we prefer to use the notation
$M^*$ because this map plays a special role in our proof.
\newline

Now we start our inductive argument.  
By Corollary \ref{structure22}, we have
$$
p_2=M_1(p_1)=\mu_2(p_1).
$$
By Theorem \ref{structure3}, we have
$$p_2 \in \widehat \psi(T_1) \cap T_2 =
\widehat \psi(T(a_1 \to b_1) \cap T(a_2 \to b_2) \subset \Sigma(b_1 \to a_2).$$
Since the map $M_1^*$ is the composition of strip maps
$$\mu_{a_2-1}, \ldots \mu_{b_1},$$
and $p_2$ belongs to all the corresponding strips, 
we have
$$M_2^*(p_2)=p_2.$$
Hence
$$
p_2=M^*_2 \circ M_1(p_1)$$
$$ = \mu_{a_2-1} \circ ... \circ \mu_1(p_0)$$
\begin{equation}
=q_{a_2-1}.
\end{equation}
By Corollary \ref{structure22}, we have
$$p_3=M_2(p_2).$$
Applying Theorem \ref{structure3} in the same was as for $p_2$, we have
$$M_3^*(p_3)=p_3.$$
Hence
$$
p_3=M_3^* \circ M_2(p_2)
$$
$$=\mu_{a_3-1} \circ ... \circ \mu_{a_2}(p_2)$$
\begin{equation}
=\mu_{a_3-1} \circ ... \circ \mu_1(p_1)=q_{a_3-1}.
\end{equation}
Continuing this way -- i.e. using induction -- we have
\begin{equation}
\label{final}
p_k=q_{a_k-1} \hskip 30 pt k=2,3,4 \ldots
\end{equation}
Equation \ref{final} takes care of both statements
of the lemma at the same time.  The point is that
$|a_{k+1}-a_k|<2n$ for any index $k$.
\endproof

\subsection{Proofs of the Main Results}

Let $\widehat \Psi$ be the first return map
to the pinwheel strip $\Sigma_1$.

We can choose a compact set $K \subset \Sigma_1$ to be
so large that any $p \in \Sigma_1-K$ has the following
property.  If $p=\mu_m(p')$, then $m=1$. If we take
indices mod $n$, we would say that
$m \equiv 1$ mod $n$.  Here, as usual, $n$ denotes
the number of sides of the nice polygon $P$
underlying all our constructions.
\newline
\newline
{\bf Proof of the Pinwheel Theorem:\/}
Suppose $p \in \Sigma_1-K$.  Suppose
first that there is some positive $k_1$ such that
$q=\widehat \Psi^{k_1}(p) \in \Sigma_1-K$. 
By the Orbit Equivalence Lemma,
$$q=\mu_{m} \circ \ldots \circ \mu_1(p).$$
From what we have said above,
$m=k_2m+1$ for some $k_2$. Hence
$q=M^{k_2}(p)$.
This establishes the first half of the unbounded
equivalence.

For the second half, suppose that
$q=M^{k_1}(p) \in \Sigma_1-K$.
We can choose $K$ large enough that the
case $k_1=1$ involves
only the analysis we did in \S \ref{easy}.
So, it suffices to consider the case when $k_1 \geq 2$.
Using the notation from the previous section, we have
$q=q_{h_1}$ for some $h_1 \geq 2n$. 
By the Orbit Equivalence Lemma, there is some
$h_2$ such that 
$h_2 \leq h_1<h_2+2n$ and
\begin{equation}
q_{h_2}=p_{h_3}=(\widehat \psi)^{h_3}(p).
\end{equation}
If we take $K$ sufficiently large, then all
$2n$ $\widehat \psi$-iterates of $q_{h_2}$
remain in the unbounded tiles of the forward partition.
This gives
$$q=q_{h_1}=\mu_{h_1} \circ  \ldots \circ \mu_{h_2+1}(q_{h_2})$$
$$=^*\widehat \psi^{h_1-h_2}(q_{h_2})
=\widehat \psi^{h_1-h_2}(p_{h_3})
=\widehat \psi^{k_2}(p).$$
Here we have set $k_2=h_1-h_2+h_3$.
The starred equality comes from the
analysis in \S \ref{easy}.
This completes the proof of the
Pinwheel Theorem.
\endproof
\newline
\noindent
{\bf Proof of Corollary \ref{iso}:\/}
Consider the $(+)$ case.
Let $U_+(P,\Psi)$ denote the set of forwards unbounded orbits
defined relative to $\Psi$.  Let
$U_+(P,M)=U_+'(P)$.  At the end of
\S \ref{easy} we remarked that there is a canonical
bijection between $U_+(P)$ and $U_+(P,\Psi)$.
The Pinwheel Theorem gives us a canonical bijection
between $U_+(P,\Psi)$ and $U_+(P,M)$.  Hence, we
get a canonical bijection between
$U_+(P)$ and $U_+(P,M)=U_+'(P)$.
The $(-)$ case follows from the $(+)$ case and symmetry.
Finally, the case
$(\pm)$ follows from the cases $(+)$ and $(-)$.
\endproof

\newpage





















==> 6diagram.tex <==

\section{Diagrams and Orientations}

Our main remaining goal is to establish
Theorem \ref{structure2}.  As a prelude
to our proof of Theorem \ref{structure2},
we discuss admissible paths in more detail.


\subsection{The Pinwheel Orientation}

We define a canonical orientation on the
spokes of a nice $n$-gon $P$.
Each spoke $S_j$ corresponds to a unique pinwheel
strip $\Sigma_j$ in the sense that the
vector $V_j$ associated to $\Sigma_j$ points
from one endpoint of $S_j$ to the other.
We orient $S_j$ by saying that ${\rm oriented\/}(S_j)=V_j$,

We say that a spoke $S_j$ is {\it special\/}
if the three spokes $S_{j-1}, S_j, S_{j+1}$ share a common vertex,
and otherwise {\it ordinary\/}.  For instance,
in Figure 2.2 the spokes $S_1$ and $S_3$ are special and the rest are
ordinary. 

\begin{lemma}
\label{orientation}
Let $\gamma$ be an admissible path of length
at least $3$.  The orientation on the 
spokes of $\gamma$ induced by the orientation on
$\gamma$ coincides with the pinwheel orientation
on all edges but the last one.  On the last
spoke, the two orientations agree if and only if
the spoke is ordinary.
\end{lemma}

\startproof
Consider a subpath of $\gamma$ that contains two spokes,
say, $S_1$ and $S_b$.  Here $b \in \{2,3,4...\}$.
Figure 6.1 shows the possible pictures, depending on $b$.

\begin{center}
\resizebox{!}{1.3in}{\includegraphics{Pix/orient.eps}}
\newline
{\bf Figure 6.1:\/} The possibilities for $b=2,3,4$.
\end{center}

In all cases, it follows from Lemma \ref{minimal1} that
there exists a minimal strip $\Sigma'$ such that $\partial \Sigma'$
contains $\partial S_1 \cup \partial S_2$.  In particular,
$\partial \Sigma'$ contains the edge $e$ shown in Figure 6.1.
But then the strip $\Sigma$ that is twice as wide as $\Sigma'$
is a pinwheel strip containing $e$ in its boundary.
Comparing Figures 1.2 and 6.1, we see that the orientation
given to $S_1$ by $\gamma$ coincides with the pinwheel
orientation on $S_1$.

It remains to describe what happens for the last spoke of $\gamma$.
The argument we just gave never uses the third property
satisfied by an admissible path.  In case the last spoke of
$\gamma$ is ordinary, we can prolong $\gamma$ by two more
spokes in such a way that the longer path $\gamma'$ satisfies
the first two properties for an admissible path.  The 
previous argument then shows that the pinwheel orientation
and the $\gamma$-induced orientations coincide the third-to-last
spoke of $\gamma'$, which is the last spoke of $\gamma$.

\begin{center}
\resizebox{!}{1.6in}{\includegraphics{Pix/orient2.eps}}
\newline
{\bf Figure 6.2:\/} Ending on a special spoke.
\end{center}

Suppose that the last spoke of $\gamma$ is special.
Just for the sake of argument, let's suppose that
the last spoke of $\gamma$ is labelled $S_2$.
Figure 6.2 shows the picture of the last two
spokes of $\gamma$ when $S_2$ is special.
In this case $e \in \Sigma_2$.  Comparing
Figures 1.2 and 6.2 we see this time that the
orientation on $S_2$ given by $\gamma$ is
$-V_j$, as claimed.
\endproof

\subsection{Diagrams for Admissible Paths}

What we describe in this section is a convenient
pictorial representation of an admissible path.
An admissible path consists of an odd number
of spokes, and we represent these by a thick
zig-zag that starts on the left.  An admissible
path skips over all the special spokes that
are not first or last. We represent these
special spokes as thinner segments.  
One might that our schematic representation
is obtained by separating out the crossings
in the admissible path to keep it embedded.
Figure 6.3 shows an actual path on the
left and our schematic representation on the right.
The schematic representation is always oriented
from top to bottom.  We have added labels to the
schematic representation to indicate the correspondence
to the actual path, but in practice we will leave
these labels off.

\begin{center}
\resizebox{!}{2.5in}{\includegraphics{Pix/schematic.eps}}
\newline
{\bf Figure 6.3:\/} Schematic representation of an admissible path.
\end{center}

One can easily read off all the admissible
subpaths of a given admissible path from our representation.
The admissible subpaths correspond to odd length 
subpaths whose edges are all thick, except for possible
for the first and last edges.  In other words, all
the spokes of an admissible path are ordinary,
except for the first and last ones.

We are going to change our terminology slightly and speak
of {\it odd admissible paths\/} and {\it even admissible paths\/}.
The odd admissible paths are precisely the paths we have been
calling just plain {\it admissible\/}.  An even admissible
path satisfies the same properties as an odd admissible
path, except that it has an even number of spokes.
We can represent even admissible paths with diagrams just
like the one in Figure 6.3.  The even admissible paths
do not correspond to admissible pairs of vertices,
but they will still prove useful for our analysis.

\end{document}


\begin{center}
\resizebox{!}{2.5in}{\includegraphics{Pix/reverse.eps}}
\newline
{\bf Figure 6.3:\/} The reverse of an admissible path
\end{center}



\end{document}


